TuringViT: Making SOTA Vision Transformers Accessible to All

Modern VLMs and VLA systems commonly adopt off-the-shelf ViTs such as SigLIP2 as visual encoders, but diverse downstream requirements in latency, temporal modeling, and VLM integration often call for customized SOTA-level ViTs. Training such encoders remains beyond the reach of much of the community, as it requires massive image-text data, while standard softmax attention makes high-resolution or dynamic-resolution pretraining prohibitively costly and often forces low-resolution pretraining followed by post-hoc adaptation. TuringViT addresses these challenges with three key designs: Turing Linear Attention (TLA) for efficient sequence modeling, VISTA-Curation to construct supervision-rich image-video training data, and native dynamic-resolution pretraining that supports flexible inputs from the start and transfers seamlessly to downstream VLMs. As a result, TuringViT outperforms leading open-source ViT baselines with only 10% of the data, achieves stronger downstream VLM performance, and delivers substantially better latency scaling on high-resolution inputs. Our scaling-law analysis further shows that TuringViT continues to improve predictably with curated data scale, far from saturation. Its fast adaptation, hardware-friendly design, and efficient deployment have made it a unified visual foundation across XPeng's AI systems. More broadly, TuringViT provides a reproducible pipeline that dramatically lowers the cost for the community to train, customize, and deploy SOTA-level ViTs, moving toward making such Vision Transformers accessible to all.

==> sec/2_related_works.tex <==
\section{Related Works}
\label{sec:related_works}


{\bf Native resolution for CLIP.} The rapid development and increasing attention of Vision-Language Models (VLMs) in recent years have also led to significant advances in visual foundation models\cite{align,clip,filip}, which play a crucial role in determining VLM performance. Contrastive Language--Image Pre-training (CLIP) \cite{clip} has emerged as a foundational model for vision-language understanding, learning a shared embedding space from large-scale image--text pairs. Its ability to perform zero-shot transfer and serve as a robust visual backbone has made it a cornerstone for many downstream VLM architectures. However, CLIP is typically trained on low-resolution images (e.g., 224$\times$224), which limits its capacity to capture fine-grained visual details. To address this, recent works have explored strategies to incorporate higher native resolutions. For instance, InternVL \cite{internvl} employs a tiling mechanism that partitions high-resolution inputs into smaller patches, enabling the model to leverage the original CLIP vision encoder without fine-tuning at higher resolutions. While effective, this approach introduces artificial cropping and relies on hand-crafted splitting strategies, which may undermine the model’s ability to learn holistic representations autonomously. Alternative methods, such as adaptive resolution scaling and dynamic patch merging, attempt to preserve both local detail and global context without rigid tiling. These limitations motivate the need for a training paradigm that supports native high-resolution processing while maintaining the model’s end-to-end learning capability.

{\bf Data curation for CLIP.} The success of contrastive vision-language models such as CLIP \cite{clip} relies heavily on the quality and scale of image--text training data. Early works curated datasets from web alt-text (e.g., Conceptual Captions \cite{conceptual_captions}), but modern models demand hundreds of millions or billions of pairs, necessitating efficient and scalable data curation pipelines. Recent works incorporate metadata or synthetic captioning to enrich alignment. MetaCLIP \cite{metaclip} introduced a data curation pipeline that balances concept coverage by leveraging metadata from external knowledge sources, achieving strong performance with significantly fewer samples. Meanwhile, models like BLIP \cite{blip} and LLaVA \cite{llava} have shown that synthetic captions generated by existing vision-language models can enhance alignment, though they introduce additional computation. With the growing scale of data, efficiency in curation---both in compute and storage---has become paramount. Techniques such as on-the-fly filtering during training, progressive data selection, and leveraging smaller proxy models for filtering have been explored to reduce overhead. Recent benchmarks like DataComp \cite{datacomp} extend these insights to large-scale multimodal pre-training, underscoring the transferability of efficient curation principles. Collectively, these works highlight that scalable, high-quality data curation is a foundational component of modern vision-language pre-training, and further advances in this direction remain essential for enabling efficient training with native high-resolution inputs.


